Possible Value Analysis based on Symbolic Lattice

We propose a new static program analysis called program behavior analysis. The analysis aims to calculate possible symbolic expressions for every variable at each program point. We design a new lattice, transfer function, and widening operator to accommodate the analysis. Furthermore, we extend the analysis to interprocedural.

==> fig/cfa.tex <==
\begin{figure}
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \begin{minted}[frame=single, fontsize=\scriptsize, breaklines, linenos, numbersep=2pt]{diff}
% @@ -238,6 +238,9 @@ int ff_vmafmotion_init(VMAFMotionData *s,
%     int i;
%     const AVPixFmtDescriptor *desc = av_pix_fmt_desc_get(fmt);

% +    if (w < 3 || h < 3)
% +        return AVERROR(EINVAL);
% +
%                     \end{minted}
%         \caption{Patch for CVE-2020-22019}
%         \label{fig:CVE-2020-22019}
%     \end{subfigure}
%     \hfill
    % \begin{subfigure}[t]{0.38\textwidth}
        \centering
        \begin{minted}[frame=single, fontsize=\scriptsize, breaklines, linenos, numbersep=2pt]{diff}
@@ -257,6 +257,9 @@ int sum(int a[], int n) {
    int i = 0;
-   int sum = 0;
+   int sum = 1;
    for (i = 0; i < n; i++)
-        sum += a[i];
+        sum *= a[i];
    return sum;
                    \end{minted}
        \caption{Refinement Example}
    % \end{subfigure}
    % \caption{Examples of patches real world projects}
    \label{fig:cfa}
\end{figure}

==> fig/refinement.tex <==
\begin{figure}
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \begin{tikzpicture}
            \node (top) at (0,3) {$\top$};
            \node (e) at (0,1) {Expression($e$)};
            \node (bot) at (0,-1) {$\bot$};
            \node (L) at (0, -2) {$L_0$};
            \node (to) at (1.5, 1) {$\longrightarrow$};
            \draw (bot) -- (e) -- (top);
        \end{tikzpicture}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \begin{tikzpicture}
            \node (top) at (0,3) {$\top$};
            \node (e) at (0,1) {Expression($e$)};
            \node (bot) at (0,-1) {$\bot$};
            \node (L) at (0, -2) {$L_1$};
            \draw (bot) -- (e) -- (top);
        \end{tikzpicture}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \begin{tikzpicture}
            \node (top) at (0,3) {$\top$};
            \node (a) at (-2,2) {$(0,1,1)$};
            \node (b) at (0,2) {$(1,0,1)$};
            \node (c) at (2,2) {$(1,1,0)$};
            \node (d) at (-2,0) {$const$};
            \node (e) at (0,0) {$mem$};
            \node (f) at (2,0) {$e$};
            \node (bot) at (0,-1) {$\bot$};
            \node (L) at (0, -2) {$L_2$};
            \draw (bot) -- (d) -- (a) -- (top) -- (b) -- (f)
            (e) -- (bot) -- (f) -- (c) -- (top)
            (d) -- (b);
            \draw[preaction={draw=white, -,line width=4pt}] (a) -- (e) -- (c);
        \end{tikzpicture}
    \end{subfigure}
    \caption{Refinement process}
    \label{fig:refinement}
\end{figure}
